PanoGRF: Generalizable Spherical Radiance Fields for Wide-baseline Panoramas

Achieving an immersive experience enabling users to explore virtual environments with six degrees of freedom (6DoF) is essential for various applications such as virtual reality (VR). Wide-baseline panoramas are commonly used in these applications to reduce network bandwidth and storage requirements. However, synthesizing novel views from these panoramas remains a key challenge. Although existing neural radiance field methods can produce photorealistic views under narrow-baseline and dense image captures, they tend to overfit the training views when dealing with \emph{wide-baseline} panoramas due to the difficulty in learning accurate geometry from sparse $360^{\circ}$ views. To address this problem, we propose PanoGRF, Generalizable Spherical Radiance Fields for Wide-baseline Panoramas, which construct spherical radiance fields incorporating $360^{\circ}$ scene priors. Unlike generalizable radiance fields trained on perspective images, PanoGRF avoids the information loss from panorama-to-perspective conversion and directly aggregates geometry and appearance features of 3D sample points from each panoramic view based on spherical projection. Moreover, as some regions of the panorama are only visible from one view while invisible from others under wide baseline settings, PanoGRF incorporates $360^{\circ}$ monocular depth priors into spherical depth estimation to improve the geometry features. Experimental results on multiple panoramic datasets demonstrate that PanoGRF significantly outperforms state-of-the-art generalizable view synthesis methods for wide-baseline panoramas (e.g., OmniSyn) and perspective images (e.g., IBRNet, NeuRay).

==> my_tex_libs/figures/fig_ab.tex <==
% \newcommand{\resultsfigwidth}{1.5in}
% \newcommand{\resultscropwidth}{0.7in}
% \renewcommand{\resultscropwidth}{0.79in}
% Define the crops here, individually for each image
% \newcommand{\cropabfirst}[1]{
%   \makecell{
%   % left bottom right top
%   % {"bbox": [226, 127, 721, 308]}
%   % {"bbox": [305, 209, 680, 264]}
%   \includegraphics[trim={305px 209px  680px 264px}, clip, width=\resultscropwidth]{#1} \\
%   % {"bbox": [4, 2, 845, 335]}
%   % {"bbox": [306, 203, 663, 254]}
%   % {"bbox": [235, 127, 714, 310]}
%   \includegraphics[trim={235px 127px 714px 310px}, clip, width=\resultscropwidth]{#1} 
%   }
% }
\newcommand{\resultsfigwidthab}{1.9in}
\newcommand{\resultscropwidthab}{0.8in}
\newcommand{\cropabfirst}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [226, 127, 721, 308]}
  % {"bbox": [305, 209, 680, 264]}
  % {"bbox": [638, 333, 290, 83]}
  % {"bbox": [592, 312, 286, 54]}
  \includegraphics[trim={592px 312px  286px 54px}, clip, width=\resultscropwidthab]{#1} \\
  % {"bbox": [4, 2, 845, 335]}
  % {"bbox": [306, 203, 663, 254]}
  % {"bbox": [235, 127, 714, 310]}
  % {"bbox": [130, 114, 688, 192]}
  \includegraphics[trim={130px 114px 688px 192px}, clip, width=\resultscropwidthab]{#1} 
  }
}

\newcommand{\cropabsecond}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [226, 127, 721, 308]}
  % {"bbox": [305, 209, 680, 264]}
  % {"bbox": [23, 134, 914, 291]}
  \includegraphics[trim={23px 134px  914px 291px}, clip, width=\resultscropwidthab]{#1} \\
  % {"bbox": [4, 2, 845, 335]}
  % {"bbox": [306, 203, 663, 254]}
  % {"bbox": [235, 127, 714, 310]}
  % {"bbox": [549, -5, 238, 280]}
  \includegraphics[trim={549px 0px 238px 275px}, clip, width=\resultscropwidthab]{#1} 
  }
}

\begin{figure*}[htbp]
\centering
\scriptsize
\begin{tabular}{@{}c@{\,\,}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\setlength{\tabcolsep}{10pt}
% \begin{tabular}{@{}c@{\,\,}c@{\,\,}c@{}c@{}c@{}c@{}}
% \begin{tabular}{ccccc}
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidthab]{results/ab_replica_wide/gt_draw/1.jpg}
% \\
% \textit{Sample 1}
% }
% & 
% \cropabfirst{results/ab_replica_wide/gt/1.jpg} &
% \cropabfirst{results/ab_replica_wide/ours_wo_stereo/1.jpg}&
% \cropabfirst{results/ab_replica_wide/ours_wo_mono/1.jpg}&

% \cropabfirst{results/ab_replica_wide/ours/1.jpg}

% \\
\makecell[c]{
\includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidthab]{results/ab_replica_wide/gt_draw/17.jpg}
\\
% \textit{Sample 2}
}
& 
\cropabsecond{results/ab_replica_wide/gt/17.jpg} &
\cropabsecond{results/ab_replica_wide/ours_wo_stereo/17.jpg}&
\cropabsecond{results/ab_replica_wide/ours_wo_mono/17.jpg}&

\cropabsecond{results/ab_replica_wide/ours/17.jpg}

\\

& Ground Truth & w/o MVS  & w/o Mono& full  
\end{tabular}
\caption{The visualization for ablation studies on Replica. }
\label{fig:res-ab}
\end{figure*}

==> my_tex_libs/figures/fig_cmp.tex <==
\newcommand{\resultsfigwidth}{1.5in}
\newcommand{\resultscropwidth}{0.75in}
% \renewcommand{\resultscropwidth}{0.79in}
% Define the crops here, individually for each image
\newcommand{\cropcmpfirst}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [218, 211, 584, 79]}
  \includegraphics[trim={218px 211px  584px 79px}, clip, width=\resultscropwidth]{#1} \\
  % {"bbox": [4, 2, 845, 335]}
  \includegraphics[trim={4px 2px 845px 335px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpsecond}[1]{
  \makecell{
  % left bottom right top
% {"bbox": [663, 100, 250, 301]}
  \includegraphics[trim={663px 110px  250px 301px}, clip, width=\resultscropwidth]{#1} \\
  % {"bbox": [4, 2, 845, 335]}
  % {"bbox": [154, 83, 787, 346]}
  \includegraphics[trim={154px 83px 787px 346px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpthird}[1]{
  \makecell{
  % left bottom right top
\includegraphics[trim={115px 108px 703px 198px}, clip, width=\resultscropwidth]{#1} \\
% {"bbox": [321, 22, 540, 327]}
  \includegraphics[trim={321px 22px 540px 327px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpforth}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [111, 149, 844, 294]}
\includegraphics[trim={111px 149px 844px 294px}, clip, width=\resultscropwidth]{#1} \\
  \includegraphics[trim={375px 4px 426px 285px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpfifth}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [111, 149, 844, 294]}
  % {"bbox": [247, 72, 571, 234]}
\includegraphics[trim={247px 72px 571px 234px}, clip, width=\resultscropwidth]{#1} \\
% {"bbox": [636, 1, 203, 326]}
  \includegraphics[trim={636px 1px 203px 326px}, clip, width=\resultscropwidth]{#1} 
  }
}




\begin{figure*}[htbp]
\centering
\scriptsize
\begin{tabular}{@{}c@{\,\,}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\setlength{\tabcolsep}{10pt}
% \begin{tabular}{@{}c@{\,\,}c@{\,\,}c@{}c@{}c@{}c@{}}
% \begin{tabular}{ccccc}
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_m3d/gt_draw/0.jpg}
% \\
% \textit{Sample 1}
% }
% & 
% \cropcmpfirst{results/cmp_m3d/gt/0.jpg} &
% \cropcmpfirst{results/cmp_m3d/ibrnet/0.png} &
% \cropcmpfirst{results/cmp_m3d/omnisyn/0.jpg} &
% \cropcmpfirst{results/cmp_m3d/neuray/0.jpg} &
% \cropcmpfirst{results/cmp_m3d/panogrf/0.jpg}

% \\
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_m3d/gt_draw/1.jpg}
% \\
% \textit{Sample 2}
% }
% & 
% \cropcmpsecond{results/cmp_m3d/gt/1.jpg} &
% \cropcmpsecond{results/cmp_m3d/ibrnet/1.png} &
% \cropcmpsecond{results/cmp_m3d/omnisyn/1.jpg} &
% \cropcmpsecond{results/cmp_m3d/neuray/1.jpg} &
% \cropcmpsecond{results/cmp_m3d/panogrf/1.jpg}
% \\
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_replica_wide/gt_draw/1.jpg}
% \\
% \textit{Sample 3}
% }
% & 
% \cropcmpthird{results/cmp_replica_wide/gt/1.jpg} &
% \cropcmpthird{results/cmp_replica_wide/ibrnet/1.png} &
% \cropcmpthird{results/cmp_replica_wide/omnisyn/1.jpg} &
% \cropcmpthird{results/cmp_replica_wide/neuray/1.jpg} &
% \cropcmpthird{results/cmp_replica_wide/panogrf/1.jpg}
\\
\makecell[c]{
\includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_replica_wide/gt_draw/6.jpg}
\\
% \textit{Sample 4}
}
& 
\cropcmpfifth{results/cmp_replica_wide/gt/6.jpg} &
\cropcmpfifth{results/cmp_replica_wide/ibrnet/6.png} &
\cropcmpfifth{results/cmp_replica_wide/omnisyn/6.jpg} &
\cropcmpfifth{results/cmp_replica_wide/neuray/6.jpg} &
\cropcmpfifth{results/cmp_replica_wide/panogrf/6.jpg}
\\

& Ground Truth & IBRNet$^{*}$~\cite{ibrnet} & OmniSyn~\cite{omnisyn}&NeuRay$^{*}$~\cite{neuray} & \sysname{} 


\end{tabular}
\caption{Qualitative comparison on Replica between IBRNet, OmniSyn, NeuRay and \sysname{}.}
\label{fig:res-cmp}
\end{figure*}

==> my_tex_libs/tables/tables_cmp.tex <==
% todo:Analysis, tables and figures.
\begin{table}
  \caption{Quantitative comparisons with baseline methods on Matterport3D. The best results are in bold.}
  \label{tab:cmp_m3d}
  \setlength\tabcolsep{1pt} % 调小列间距
  \centering
  % \resizebox*{1.0\linewidth}{!}{
  \begin{tabular}{cccccccccc}
    \toprule
    baseline & \multicolumn{3}{c}{1.0m} & \multicolumn{3}{c}{1.5m} & \multicolumn{3}{c}{2.0m} \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}    \cmidrule(lr){8-10}
    method & WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ &  WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ &  WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$\\
    % \midrule
    \cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}    \cmidrule(lr){8-10}
    S-NeRF  & 15.25&0.579&0.546&14.16&0.563&0.580&13.13&0.523&0.607      \\
    OmniSyn &22.90&0.850&0.244&20.31&0.790&0.317&18.91&0.761&0.354\\
    IBRNet$^{*}$  & 25.72&0.855&  0.258 &21.69&0.751&0.382 &20.04&0.706&0.431     \\
    NeuRay$^{*}$ & 24.92&0.832&0.260&21.92&0.766&0.347&19.85&0.715&0.407  \\
    \sysname{} &{\bfseries27.12}&{\bfseries0.876}&{\bfseries0.195}&{\bfseries23.38}&{\bfseries0.811}&{\bfseries0.282}&{\bfseries20.96}&{\bfseries0.761}&{\bfseries0.352} \\
    \bottomrule
  \end{tabular}
  % }
\end{table}


\begin{table}
  \caption{Quantitative comparison with baseline methods on Replica and Residential Dataset}
  \label{tab:cmp_replica}
  \setlength\tabcolsep{4pt} % 调小列间距
  \centering
  \begin{tabular}{ccccccccc}
    \toprule
    Dataset & \multicolumn{4}{c}{Replica (1.0m)}&\multicolumn{4}{c}{Residential (about 0.3m)}\\

    \cmidrule(r){1-1}    \cmidrule(r){2-5} \cmidrule(r){6-9}
    method & PSNR$\uparrow$ & WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$\\
    % \midrule
    \cmidrule(r){1-1}    \cmidrule(r){2-5} \cmidrule(r){6-9}
    S-NeRF & 16.91 & 16.10 &0.723 & 0.443& 23.06 & 22.47 & 0.741 & 0.435\\
    OmniSyn & 23.91 & 23.17 & 0.898&0.189&-&-&-&-\\
    IBRNet$^*$ & 23.35 & 22.65 & 0.854 &0.291& 22.95 & 22.47 & 0.735 &0.498 \\
    NeuRay$^*$ & 26.62 & 25.90 & 0.899 &0.187 & 23.01 & 22.38 & 0.753 &0.427\\
    \sysname{}&{\bfseries30.08} &{\bfseries29.22}  & {\bfseries0.937} &{\bfseries0.134}&{\bfseries31.64} &{\bfseries31.03}  & {\bfseries0.909} &{\bfseries0.207}\\
    \bottomrule
  \end{tabular}
\end{table}

